Varuna: Scalable, Low-cost Training of Massive Deep Learning Models

Systems for training massive deep learning models (billions of parameters) today assume and require specialized "hyper-clusters": hundreds or thousands of GPUs wired with specialized high-bandwidth interconnects such as NV-Link and Infiniband. Besides being expensive, such dependence on hyper-clusters and custom high-speed inter-connects limits the size of such clusters, creating (a) scalability limits on job parallelism; (b) resource fragmentation across hyper-clusters. In this paper, we present Varuna, a new system that enables training massive deep learning models on commodity networking. Varuna makes thrifty use of networking resources and automatically configures the user's training job to efficiently use any given set of resources. Therefore, Varuna is able to leverage "low-priority" VMs that cost about 5x cheaper than dedicated GPUs, thus significantly reducing the cost of training massive models. We demonstrate the efficacy of Varuna by training massive models, including a 200 billion parameter model, on 5x cheaper "spot VMs", while maintaining high training throughput. Varuna improves end-to-end training time by up to 18x compared to other model-parallel approaches and up to 26% compared to other pipeline parallel approaches. The code for Varuna is available at https://github.com/microsoft/varuna.

==> related.tex <==
\section{Related Work}
\label{sec-related}

In this section, we review work closely related to training massive models.

\noindent
{\bf Inter-layer/pipeline parallelism.}
Inter-layer or pipeline parallelism has been used in many systems~\cite{Gpipe,pipedream,pipemare} but in different ways. Gpipe~\cite{Gpipe} was one of the first systems to use pipeline partitioning to split a large model (6 billion parameters) among a number of GPUs. Gpipe follows the synchronous SGD semantics where gradients are applied synchronously at the end but this can result in "bubble overhead" where many pipeline stages are stalled. Gpipe uses micro-batches to reduce the pipeline overhead but assumes that the user provides a partitioned model as input. \varuna\ follows the synchronous SGD semantics of Gpipe but automatically partitions the user's model to minimize the pipeline overhead.

Unlike Gpipe, Pipedream achieves 100\% pipeline utilization in steady state. However, to achieve this, Pipedream sacrifices synchronous SGD semantics as the parameter updated is delayed. Further, Pipedream has to keep a copy of the parameters used in the forward pass so that the same parameters can be used in the backward pass, and this increases memory overhead substantially compared to Gpipe and \varuna. While Pipedream achieves desired accuracy for computer vision tasks, the lack of synchronous SGD semantics results in it failing to converge for language translation tasks such as IWSLT/WMT~\cite{pipemare}.


Pipemare~\cite{pipemare} deviates further from synchronous SGD semantics by using asynchronous pipeline-parallel training. Thus, unlike Pipedream, Pipemare does not keep extra copy of parameters and allows the backward pass to update a different set of parameters than that used by the corresponding forward pass! This allows Pipemare to avoid the memory overhead of Pipedream while retaining full utilization. However, Pipemare's asynchronous semantics can result in errors during training. Thus, Pipemare introduces new techniques to adjust for the asynchronous training discrepancies. While the authors show that Pipemare has better convergence than Pipedream, they evaluate only on smaller models (12-layer transformer with 110 million parameters). It is not clear if asynchronous training with their correction techniques will work on massive models like BERT-large and GPT-2.

\noindent
{\bf Intra-layer parallelism.}
Mesh tensorflow~\cite{meshtf}, Megatron~\cite{shoeybi2019megatron}, and Turing~\cite{Turing} adopt the intra-layer parallelism to scale to large models with the largest being Turing's 17 billion parameter model. However, as discussed earlier, these approaches require high bandwidth and low latency connectivity since the communication is in the critical path and cannot be overlapped. Thus, for efficiency, Megatron and Turing models use DGX-2s with the model partitioned only within the DGX-2 so that the communication can benefit from the 2.4 Tbps NVlink connectivity.


 
\noindent
{\bf Memory optimizations.}
Gradient checkpointing~\cite{checkpointing, checkmate} is a well-known technique to reduce GPU memory usage, where the activations are recomputed for the backward pass. 
Activations can also be stashed in CPU memory and brought back to GPU when needed instead of performing the recomputation~\cite{geeps} but this can incur substantial overhead~\cite{cpumemoverhead}. Activations can also be compressed to reduce their memory usage and decompressed before backward pass~\cite{gist}. RELU activations~\cite{relu} are highly compressible but large models like BERT use GELU activations~\cite{gelu} are not compressible. Finally,  ZeRO/DeepSpeed~\cite{zero} optimizes memory usage in data-parallel training by sharding the redundant state among the replicas, thereby allowing substantial savings in memory usage. \varuna\ currently uses gradient checkpointing with recomputation but can benefit from some of these other memory optimizations as well.

\noindent
{\bf Resource elasticity.} Recent frameworks such as PyTorch Elastic~\cite{elastic} and MXNet Dyanmic~\cite{mxnetdl} support training over dynamic set of resources. However, these frameworks assume that user scripts are configured with the right parameters for all available resources. Proteus~\cite{harlap2017proteus} supports flexible training on dynamic set of resources by simply splitting the data evenly across all nodes while authors in~\cite{reselastic} support auto-scaling in data-parallel training by profiling the incremental speedup of using more resources for replicas and automatically scaling resources until the marginal utility drops below the marginal cost of additional resources. Unlike~\cite{reselastic} and ~\cite{harlap2017proteus}, scaling in \varuna\ is two-dimensional, i.e., given a set of resources, \varuna\ needs to determine both the number of pipeline stages as well as number of data-parallel replicas and identify the best configuration that maximizes performance.

\noindent
{\bf Training on Spot VMs} Proteus\cite{harlap2017proteus} enables training machine learning models over flexible set of spot and dedicated VMs by organizing resources into tiers of expected reliability, and maintaining states on few reliable nodes while exploiting spot VMs as worker nodes.  However, this approach is specific to parameter server framework and does not scale with large cluster and model sizes. 

==> scaling.tex <==
\section{Scaling Limits of DLT jobs}
\label{sec-scaling}


In this paper, we are interested in training massive models, with hundreds of millions to tens of billions of parameters. These are typical sizes of state-of-the-art natural language processing (NLP) models today. Typically, computer vision models are smaller (have tens of millions of parameters). Thus, we focus on massive NLP models in this paper.

\subsection{Compute}

On a 16GB V100 GPU, training performance for BERT-large using half-precision is about 26.6 examples/sec~\cite{nvidiabert}.  Training a BERT-large model takes 1 million iterations with a mini-batch of 256 examples~\cite{bert-large}. Thus, to train BERT-large on a single V100 would take about 256 million/26.6 seconds or 111 days of training! 

One can reduce time-taken by using data-parallel but even on 64 TPUv2 chips, BERT-large takes 4 days~\cite{bert-large}. Thus, training these models can be expensive. Authors in~\cite{trainingcost} estimate that
a single BERT-large training run costs \$10K with a fully-loaded cost of \$200K that accounts for
multiple runs with hyper-parameter tuning. As models get larger, the compute requirements and costs increase further. For example, a 1.5 billion parameter model would cost \$80K for a single training run~\cite{trainingcost}. Thus, the use of low-priority VMs is critical to reduce the cost of
training these large models.

\subsection{Memory}

For large models, limited GPU memory poses a significant constraint. Consider a model with N parameters. These models are trained in half-precision to maximize compute performance and thus require N*2 bytes to store model parameters and N*2 bytes to store gradients. In addition, a full-precision master copy of the parameters of size N*4 bytes is maintained for convergence~\cite{mixedprecision}. Finally, these models are trained using the Adam optimizer~\cite{adam}, which maintains the first and second moments of parameters in full precision, requiring N*8 bytes. Thus, a model with N parameters requires a minimum of N*16 bytes of memory for storing the parameters and optimizer state.
An approach like Pipedream~\cite{pipedream} uses multiple copies of parameters to reduce staleness effects in their pipeline. This implies that Pipedream would need to store multiple copies of N*16 bytes, which can be prohibitive for massive NLP models.


In addition, to do the backward pass, one needs the intermediate outputs of the forward computation, called the activations. The activation size depends on the model and batch size used. For NLP models like BERT-large, the activation size is roughly N bytes per input example. Larger batch size is more compute-efficient, but also implies larger memory needs; a batch size of 16 implies N*16 bytes of memory required for the activations alone, which can be substantial when N is large.

One technique to save memory is called activation or gradient checkpointing~\cite{checkpointing}. The idea is to discard the activations during the forward pass and recompute the activations just before its backward pass. 
Gradient checkpointing reduces efficiency since the forward pass is performed twice. Since forward pass takes about one-third of the iteration compute, this adds about 33\% overhead. However,  checkpointing also allows much larger batch sizes to be used and this could improve compute  efficiency by increasing parallelization,

\subsection{Network}

While data-parallel training reduces training time by executing iterations in parallel, it typically does not achieve linear scaling because of the overhead of the all-reduce stage.  The all-reduce stage requires exchanging gradients of size N*2 bytes between the replcias. When the data-parallel is executed over large number of replicas (100s or more), half-precision resolution may be insufficient, in which case all-reduce is performed over full precision, requiring N*4 bytes of exchange. In either case, the network bandwidth requirement increases linearly with model size. Thus, for large models, the all-reduce phase quickly becomes a bottleneck over low-priority VMs with 40Gbps NICs (with switch-level bottlenecks)


In the case of model-parallelism, intra-layer partitioning requires sufficient bandwidth for input activations to be sent to the next partition (and gradients in the backward pass). For BERT-large, this is only about 512KB per input example. 
On the other hand, with inter-layer partitioning as in Megatron~\cite{shoeybi2019megatron}, the matrix-multiplication computation in the forward and backward passes are split between multiple GPUs. Thus, this requires a synchronous all-reduce of N*2 bytes for every such multiplication, necessitating low latency/jitter and high bandwidth communication. Megatron is typically trained by partitioning within a DGX-2, where NVlink provides 2.4~Tbps of bandwidth.
